Deep Stochastic Kinematic Models for Probabilistic Motion Forecasting in Traffic

In trajectory forecasting tasks for traffic, future output trajectories can be computed by advancing the ego vehicle's state with predicted actions according to a kinematics model. By unrolling predicted trajectories via time integration and models of kinematic dynamics, predicted trajectories should not only be kinematically feasible but also relate uncertainty from one timestep to the next. While current works in probabilistic prediction do incorporate kinematic priors for mean trajectory prediction, _variance_ is often left as a learnable parameter, despite uncertainty in one time step being inextricably tied to uncertainty in the previous time step. In this paper, we show simple and differentiable analytical approximations describing the relationship between variance at one timestep and that at the next with the kinematic bicycle model. In our results, we find that encoding the relationship between variance across timesteps works especially well in unoptimal settings, such as with small or noisy datasets. We observe up to a 50% performance boost in partial dataset settings and up to an 8% performance boost in large-scale learning compared to previous kinematic prediction methods on SOTA trajectory forecasting architectures out-of-the-box, with no fine-tuning.

==> sections/method_old.tex <==


\section{Simulation State Inference from Trajectory Data}
TODO

\section{Trajectory Forecasting with Car-Following Model Priors}

We propose a method for integrating car-following model priors into transformer-based trajectory forecasting models, with the goal being to guide early stage deep learning with dynamics provided by differentiable traffic simulation for faster convergence. 

\subsection{Modified Gaussian Mixture Model Head}
Current state-of-the-art solution for trajectory forecasting and agent simulation tasks related to autonomous driving adopt a transformer encoder-decoder architecture, which can be illustrated generically in Figure~\ref{fig:system-diagram}. 
In these architectures, a scene encoder network extracts scene context features representing both agent and map features. 
Those features then act as the keys and values for the autoregressive rollouts of scene decoder layers. 
Using key and values from the scene encoder, the scene decoder then produces query features that are used for trajectory prediction by the Gaussian Mixture Model (GMM) head network. 
From previous works~\cite{shi2022motion, pmlr-v100-chai20a, varadarajan_multipathplusplus22, chen2023traj, wang2023multiverse}, the GMM model predicts properties of the distribution of possible positions $\left(\mu_x, \mu_y, \sigma_x, \sigma_y, \rho \right)$ for each time step, with $\mathcal{K}$ candidate distributions. 
These candidate distributions are merged into a single probability distribution $P$ representing the agent's position $o \in \mathbb{R}^2$ at time step $i$ by the following: 

\begin{align*}
    P^j_i(o) = \sum^K_{k=1} p_k \cdot \mathcal{N}_k\left(o_x - \mu_x, \sigma_x;o_y - \mu_y, \sigma_y; \rho\right)
\end{align*}

Then, predicted trajectories are extracted via the expected values of such distributions for each timestep. 

In this formulation, the network's search space is unconstrained during training and may inevitably propose candidate solutions which are either completely unrealistic or impossible. 
Simple relationships between one vehicle and the one in front of it are left to the model to capture through the input data. 

We propose to predict the estimated car-following parameters of each vehicle in addition to x-y positions. In other words, the network will also predict a mean and variance for each parameter listed in Table~\ref{tab:idm_definitions}. 
% To be explicit, the resulting output distribution then becomes:

% \begin{align*}
%     P^j_i(o, v_0, T, a, b, \sigma) = \sum^K_{k=1} p_k \cdot \mathcal{N}_k \left( & o_x - \mu_x, \sigma_x;\\
%     & o_y - \mu_y, \sigma_y;\\
%     & v_0 - \mu_{v_0}, \sigma_{v_0};\\
%     & T - \mu_{T}, \sigma_{T};\\
%     & a - \mu_{a}, \sigma_{a};\\
%     & b - \mu_{b}, \sigma_{b}; \rho \right)
% \end{align*}

\subsection{CFM-Consistent Trajectory Formulation}

We compare the car-following parameters estimated from historical trajectory data to the output of the GMM, which includes a candidate position at the next time step and estimations of each CFM parameter for that time step. 
To do this, we represent previous trajectories as a series of simulation states in a differentiable simulator where each vehicle has a unique set of CFM parameters. 
In parallel with trajectory predictions from the GMM head network, the differentiable simulator uses the predicted CFM parameters to produce a trajectory ``prediction" based on the next time step via regular simulation, or Euler time integration. 
Given that the timestep between trajectory predictions is sufficiently small, the difference between the simulated trajectory and the predicted trajectory should not be too large. 

Given two predicted positions via both the differentiable traffic simulator $\hat{Y}_{sim}$, which is only governed by a CFM, and the trajectory forecasting network $\hat{Y}_{net}$, we then formulate the predicted trajectory as a weighted sum between the simulated distribution and the predicted distribution, $P = \alpha P_{net} + (1 - \alpha) P_{sim}$, where $P_{sim}$ assumes similar variance as the network distribution. 
The hyperparameter $\alpha$ representing the weight of the network prediction is determined by the cosine similarity of the CFM parameters predicted by the GMM and the CFM parameters estimated through the historical trajectory. 
As the CFM parameters predicted by the GMM align with that of the trajectory which already occurred, the predicted trajectory will be determined mostly by the position prediction of the GMM directly. 

In early stages of training, we can expect that the cosine similarity between predicted and historical CFM parameters will be quite large; thus the predicted trajectory will be influenced heavily by the differentiable simulator and backpropagated to the network via CFM parameters. As CFM predictions become more accurate and hyperparameter $\alpha$ approaches one, learning eventually reduces to that of a standard transfomer-based trajectory forecasting network. In other words, the differentiable traffic simulator constrains parameter search at early stages of learning via backpropagation through differentiable simulation, then dynamically hands off learning to the network as predictions become closer to car-following behavior. Since differentiable traffic simulation cannot be involved directly as a ground truth for trajectory paths, we instead use it to guide high-level learning.

\subsection{Training Loss}
For each decoder layer, a loss is computed based on the Gaussian Negative-Likelihood objective to increase the likelihood of the ground truth trajectory in addition to the value $\gamma\alpha$, which represent the cosine similarity between predicted CFM parameters and historical CFM parameters, weighted by hyperparameter $\gamma$. The final loss represents the sum of all decoder losses. 




% see section Multimodal motion prediction with Gaussian Mixture Model from Motion Transformer paper. 

% result may not directly translate. Might have to borrow inspiration from the multiverse transformer to update simulation features in autoregressive decoder 


